Table Question Answering for Low-resourced Indic Languages

TableQA is the task of answering questions over tables of structured information, returning individual cells or tables as output. TableQA research has focused primarily on high-resource languages, leaving medium- and low-resource languages with little progress due to scarcity of annotated data and neural models. We address this gap by introducing a fully automatic large-scale tableQA data generation process for low-resource languages with limited budget. We incorporate our data generation method on two Indic languages, Bengali and Hindi, which have no tableQA datasets or models. TableQA models trained on our large-scale datasets outperform state-of-the-art LLMs. We further study the trained models on different aspects, including mathematical reasoning capabilities and zero-shot cross-lingual transfer. Our work is the first on low-resource tableQA focusing on scalable data generation and evaluation procedures. Our proposed data generation method can be applied to any low-resource language with a web presence. We release datasets, models, and code (https://github.com/kolk/Low-Resource-TableQA-Indic-languages).

==> prompts/gpt_prompt.tex <==
\begin{llmPrompt}[title={Prompt \thetcbcounter: GPT-3.5 Prompt}, label=prompt:gpt]
    % {\bng Aapin Ekjn sHayk sHkarii iJin baNNGla pResh/nr Ut/tr edn baNNGla eTibl ethek baNNGlay Ut/tr eTibl oitir ker.} \small m {\bng sair EbNNG} \small tealn {\bng klamguilr EkiT eTibl inm/nilikht pYoaTaer/n elkha Hey:} <{\bng klam}> {\bng eTibl eHDar} <{\bng era 1}> {\bng man  1,1 . man 1,2 .} ... {\bng man 1,}\small \textcolor{teal}{n <}{\bng era 2}> {\bng man 2,1 .} ... <{\bng era} \small m> {\bng man} \small m,{\bng1 . man} \small m,{\bng 2 .} ... {\bng . man} \small m,n
    

    % {\bng UdaHrN:}

    % {\bng 1) pRsh/n: kTa isheranam kaUn/TDaUn?} <{\bng klam}>{\bng bchr . isheranam . bhuimka} <{\bng ra 1}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT} ... <{\bng era 13}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn }<{\bng era 14}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn} <{\bng era 15}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn}
    
    % {\bng Ut/tr:} <{\bng klam}>{\bng gNna(`isherinam`) }<{\bng era 1}> {\bng3}
    
    % {\bng 2) pRsh/n: kTa bcher isherinam sii ena Ibhl?} <{\bng klam}> {\bng  bchr . isheranam . bhuimka} <{\bng era 1}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 2}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 3}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }... 
    
    % {\bng Ut/tr:} <{\bng klam}> {\bng gNna(`bchr`)} <{\bng era 1}> {\bng  3}
    \begin{bengali}
    আপনি একজন সহায়ক সহকারী যিনি বাংলা প্রশ্নের উত্তর দেন বাংলা টেবিল থেকে বাংলায় উত্তর টেবিল তৈরি করে। m সারি এবং n কলামগুলির একটি টেবিল নিম্নলিখিত প্যাটার্নে লেখা হয়ে: <কলাম> টেবিল হেডার <রো  ১> মান ১,১ | মান ১,২ | .... | মান ১,n <রো  ২> মান ২,১ | .... <রো m> মান m,১ | মান m,২ | .... | মান m,n 
    
    উদাহরণ:
    
  ১) প্রশ্ন: কটা শিরোনাম কাউন্টডাউন? <কলাম> বছর | শিরোনাম | ভূমিকা <রো ১> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ২> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৩> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৪> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৫> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৬> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৭> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৮> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৯> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ১০> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১১> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১২> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১৩> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৪> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৫> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন
 
   উত্তর: <কলাম> গণনা(`শিরোনাম`) <রো ১> ৩
   
 
 ২) প্রশ্ন: কটা বছরে শিরোনাম সি নো ইভল? <কলাম> বছর | শিরোনাম | ভূমিকা <রো ১> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ২> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৩> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৪> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৫> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৬> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৭> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৮> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৯> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ১০> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১১> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১২> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১৩> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৪> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৫> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন
 
   উত্তর: <কলাম> গণনা(`বছর`) <রো ১> ৩
    \end{bengali}
\end{llmPrompt}



==> prompts/llm_prompt.tex <==
\begin{llmPrompt}[title={Prompt \thetcbcounter: 2-Shot ICL Prompt}, label=prompt:llm]
    {\bng Aapin Ekjn sHayk sHkarii iJin baNNGla pResh/nr Ut/tr edn baNNGla eTibl ethek baNNGlay Ut/tr eTibl oitir ker.} \small m {\bng sair EbNNG} \small n {\bng klamguilr EkiT eTibl inm/nilikht pYoaTaer/n elkha Hey:} <{\bng klam}> {\bng eTibl eHDar} <{\bng era 1}> {\bng man  1,1 . man 1,2 .} ... {\bng man 1,}\small n <{\bng era 2}> {\bng man 2,1 .} ... <{\bng era} \small m> {\bng man }\small m,{\bng1 . man }\small m,{\bng 2 .} ... {\bng . man} \small m,n

    \vspace{10pt}
    {\bng UdaHrN:}
    \vspace{10pt}

    {\bng 1)} \textbf{{\bng pRsh/n:}} {\bng kTa isheranam kaUn/TDaUn?} <{\bng klam}> {\bng  bchr . isheranam . bhuimka} <{\bng era 1}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 2}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 3}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 4}> \small 2010 {\bng . mYoakgRabar . TYoaNNGkar luitJ  }<{\bng era 5}> \small 2010 {\bng . mYoakgRabar . TYoaNNGkar luitJ} <{\bng era 6}> \small 2010 {\bng . mYoakgRabar . TYoaNNGkar luitJ }<{\bng era 7}> \small 2014 {\bng . s/kuib-eDa! ebslmYoainya ims/Tir . inej} <{\bng era 8}> \small 2014 {\bng . s/kuib-eDa! ebslmYoainya ims/Tir . inej }<{\bng era 9}> \small 2014 {\bng . s/kuib-eDa! ebslmYoainya ims/Tir . inej }<{\bng era 10}> \small 2014 {\bng . sii ena Ibhl 2 . ejkb guD naIT }<{\bng era 11}> \small 2014 {\bng . sii ena Ibhl 2 . ejkb guD naIT }<{\bng era 12}> \small 2014 {\bng . sii ena Ibhl 2 . ejkb guD naIT }<{\bng era 13}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn }<{\bng era 14}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn} <{\bng era 15}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn}

    \vspace{10pt}
{\bng Ut/tr: }<{\bng klam}> {\bng gNna(`isherinam`) }<{\bng era 1}> {\bng 3}


\vspace{20pt}

{\bng 2) pRsh/n: kTa bcher isherinam sii ena Ibhl?} <{\bng klam}> {\bng  bchr . isheranam . bhuimka} <{\bng era 1}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 2}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 3}> \small 2006 {\bng . is ena Ibhl . ejkb guD naIT }<{\bng era 4}> \small 2010 {\bng . mYoakgRabar . TYoaNNGkar luitJ  }<{\bng era 5}> \small 2010 {\bng . mYoakgRabar . TYoaNNGkar luitJ} <{\bng era 6}> \small 2010 {\bng . mYoakgRabar . TYoaNNGkar luitJ }<{\bng era 7}> \small 2014 {\bng . s/kuib-eDa! ebslmYoainya ims/Tir . inej} <{\bng era 8}> \small 2014 {\bng . s/kuib-eDa! ebslmYoainya ims/Tir . inej }<{\bng era 9}> \small 2014 {\bng . s/kuib-eDa! ebslmYoainya ims/Tir . inej }<{\bng era 10}> \small 2014 {\bng . sii ena Ibhl 2 . ejkb guD naIT }<{\bng era 11}> \small 2014 {\bng . sii ena Ibhl 2 . ejkb guD naIT }<{\bng era 12}> \small 2014 {\bng . sii ena Ibhl 2 . ejkb guD naIT }<{\bng era 13}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn }<{\bng era 14}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn} <{\bng era 15}> \small 2016 {\bng . kaUn/TDaUn . elh etRuainn}

\vspace{10pt}
{\bng Ut/tr:} <{\bng klam}> {\bng gNna(`bchr`)} <{\bng era 1}> {\bng  3}
\end{llmPrompt}

 %    আপনি একজন সহায়ক সহকারী যিনি বাংলা প্রশ্নের উত্তর দেন বাংলা টেবিল থেকে বাংলায় উত্তর টেবিল তৈরি করে।m সারি এবং n কলামগুলির একটি টেবিল নিম্নলিখিত প্যাটার্নে লেখা হয়ে: <কলাম> টেবিল হেডার <রো  ১> মান ১,১ | মান ১,২ | .... | মান ১,n <রো  ২> মান ২,১ | .... <রো m> মান m,১ | মান m,২ | .... | মান m,n 
    
 %    উদাহরণ:
    
 % ১) প্রশ্ন: কটা শিরোনাম কাউন্টডাউন? <কলাম> বছর | শিরোনাম | ভূমিকা <রো ১> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ২> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৩> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৪> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৫> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৬> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৭> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৮> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৯> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ১০> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১১> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১২> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১৩> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৪> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৫> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন
 
 %   উত্তর: <কলাম> গণনা(`শিরোনাম`) <রো ১> ৩
   
 
 % ২) প্রশ্ন: কটা বছরে শিরোনাম সি নো ইভল? <কলাম> বছর | শিরোনাম | ভূমিকা <রো ১> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ২> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৩> 2006 | সি নো ইভল | জেকব গুড নাইট <রো ৪> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৫> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৬> 2010 | ম্যাকগ্রাবার | ট্যাংকার লুতিয <রো ৭> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৮> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ৯> 2014 | স্কুবি-ডো! রেসলম্যানিয়া মিস্টরি | নিজে <রো ১০> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১১> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১২> 2014 | সী নো ইভল ২ | জেকব গুড নাইট <রো ১৩> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৪> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন <রো ১৫> 2016 | কাউন্টডাউন | লেঃ ক্রোনিন
 
 %   উত্তর: <কলাম> গণনা(`বছর`) <রো ১> ৩
 %    \end{bengali}

==> tables/hindiTabQA.tex <==
\begin{table}[!t]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l ccccc}
\toprule
\textbf{Train} & \textbf{Model} & \textbf{Tab} &  \textbf{Row} &  \textbf{Col} &  \textbf{Cell} \\
\midrule
\multirow{3}{*}{ICL}  & GPT-3.5  & $8.20$ & $10.29$ & $7.10$ & $9.81$\\
& GPT-4  & $11.11$ & $21.49$ & $11.76$ & $20.84$\\
& OpenHathi & $0.00$ & $0.11$ & $0.37$ & $0.74$\\
\midrule
\multirow{2}{*}{FT} & HiTQA-mBart & $28.93$ & $39.49$ & $28.93$ & $39.42$ \\
& HiTQA-BnTQA & $\textbf{41.32}$ & $\textbf{47.26}$ & $\textbf{41.32}$ & $\textbf{47.26}$ \\
\bottomrule
\label{tab:hitabqa}
\end{tabular}
}
\caption{Scores (\%) of HindiTabQA models on test set.}
\label{tab:hitabqa}
\end{table}


% \begin{table}[!t]
% \centering
% \label{tab:generalization_results}
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{ll cccc|cccc}
% \toprule
% \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{Hindi} & \multicolumn{4}{c}{Odia} \\
% & & \textbf{Tab} &  \textbf{Row} &  \textbf{Col} &  \textbf{Cell} &  \textbf{Tab} &  \textbf{Row} &  \textbf{Col} &  \textbf{Cell}\\
% \midrule
% \multirow{3}{*}{ICL}  & GPT-3.5  & $8.20$ & $10.29$ & $7.10$ & $9.81$\\
% & GPT-4  & $11.11$ & $21.49$ & $11.76$ & $20.84$\\
% & OpenHathi & $0.00$ & $0.11$ & $0.37$ & $0.74$\\
% \midrule
% \multirow{2}{*}{FT} & HiTQA-mBart & $28.93$ & $39.49$ & $28.93$ & $39.42$ \\
% & HiTQA-BnTQA & $\textbf{41.32}$ & $\textbf{47.26}$ & $\textbf{41.32}$ & $\textbf{47.26}$ \\
% \bottomrule
% \label{tab:hitabqa}
% \end{tabular}
% }
% \caption{Scores (\%) of HindiTabQA models on test set.}
% % \vspace*{-2\baselineskip}
% \end{table}

==> tables/hitqa_example_finetuned_models.tex <==
\if0
\begin{flushright}
    \textbf{HiTabQA-mBart}:
    {\small
    \resizebox{0.25\textwidth}{!}{
    \begin{tabular}{p{5cm}c}
    \hline
    \makecell{{\bng nam} (\emph{Name)}} \\
    \hline
     \makecell{{\bng maIekl s/kubala} (\emph{Michael Skubala)}} \\
     \makecell{{\bng els irD} (\emph{Les Reed)}} \\
      \hline
    \end{tabular}
    }}
    \end{flushright}
\fi    
\begin{center}
    \begin{tabular}{l}
        \hline
        \makecell[l]{{\bng nam} (\emph{Name)}} \\
        \hline
        \makecell[l]{{\bng maIekl s/kubala} (\emph{Michael Skubala)}} \\
        \makecell[l]{{\bng els irD} (\emph{Les Reed)}} \\
        \hline
    \end{tabular}
\end{center}

==> tables/main_results_all_lang.tex <==
\begin{table*}[!t]
% \centering
\setlength{\tabcolsep}{0.7mm}
\resizebox{0.75\textwidth}{!}{
\begin{tabularx}{1\textwidth}{l rrrr|rrrr|rrrr|rrrr|rrrr}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{Bengali (Bn)} & \multicolumn{4}{c}{Hindi (Hi)} & \multicolumn{4}{c}{Odia (Or)} & \multicolumn{4}{c}{Telugu (Te)} & \multicolumn{4}{c}{Marathi (Mr)}
\\
\cmidrule(r){2-5}
\cmidrule{6-9}
 & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}  & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell} 
 & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}
 & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}
 & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}\\
\midrule
 En2X-mBart  &  $0.00$ & $4.73$ & $0.00$ & $4.73$ \\
 TableLlama   & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
 X-Llama & $0.69$ & $1.77$ & $0.69$ & $1.4$ & $0.00$ & $0.11$ & $0.37$ & $0.74$ \\
 GPT-3.5 & $6.04$ & $10.06$ & $9.12$ & $9.84$ & $8.20$ & $10.29$ & $7.10$ & $9.81$ \\
 GPT-4 & $26.83$ & $\textbf{38.67}$ & $26.74$ & $\textbf{36.51}$ & $11.11$ & $21.49$ & $11.76$ & $20.84$ \\ 
 
 \midrule
\textbf{X-TQA-llama} & $9.41$ & $12.35$ & $9.85$ & $11.87$  & $--$ & $--$ & $--$ & $--$  & $--$ & $--$ & $--$ & $--$  & $--$ & $--$ & $--$ & $--$ \\
\textbf{X-TQA-mBart} & $\textbf{35.88}$ & $33.16$ & $\textbf{35.88}$ & $33.16$  & $28.93$ & $39.49$ & $28.93$ & $39.42$ & $--$ & $--$ & $--$   & $--$ & $--$ & $--$ & $--$ \\
\textbf{X-TQA-M2M} & $45.31$ & $58.07$ & $45.29$ & $58.04$ & $28.05$ & $34.55$ & $--$ & $--$  & $--$ & $--$ & $--$ & $--$   & $--$ & $--$ & $--$ & $--$  & $--$ & $--$ & $--$ & $--$  \\ 
\bottomrule
\end{tabularx}
}
\caption{Baseline and X-TabQA models' scores where X is the low-resourced language}
\label{tab:bengali_results_all_lang}
\end{table*}


==> tables/main_results_test_set.tex <==
\begin{table*}[!t]
\centering
\small
\begin{tabularx}{1\textwidth}{lrrrr rrrr}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{Validation Set scores (\%)} & \multicolumn{4}{c}{Test Set scores (\%)} \\ 
\cmidrule(r){2-5}
\cmidrule{6-9}
 & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}  & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell} \\
\midrule
 En2Bn-mBart  &  $0.05$ & $3.06$ & $0.20$ & $3.07$ & $0.00$ & $4.73$ & $0.00$ & $4.73$\\
 OdiaGenAI-bn  & $0.00$ & $3.89$ & $0.00$ & $3.89$ & $0.69$ & $1.77$ & $0.69$ & $1.4$2 \\
 TableLlama    & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
 GPT-3.5 & $1.14$ & $4.81$ & $1.67$ & $5.14$ & $6.04$ & $10.06$ & $9.12$ & $9.84$ \\
 GPT-4 & $0.00$ & $13.57$ & $5.43$ & $14.65$ & $26.83$ & $\textbf{38.67}$ & $26.74$ & $\textbf{36.51}$ \\
\midrule
\textbf{BnTQA-llama} & $\textbf{60.08}$ & $\textbf{68.30}$ & $\textbf{60.47}$ & $\textbf{68.30}$ & $9.41$ & $12.35$ & $9.85$ & $11.87$  \\
\textbf{BnTQA-mBart} & $56.63$  & $64.1$ & $56.79$ & $64.31$ & $\textbf{35.88}$ & $33.16$ & $\textbf{35.88}$ & $33.16$   \\
\textbf{BnTQA-M2M} & $45.31$ & $58.07$ & $45.29$ & $58.04$ & $28.05$ & $34.55$ & $28.05$ & $34.55$ \\ 
\bottomrule
\end{tabularx}
% }
\caption{Baseline and BanglaTabQA models' scores.}
\label{tab:bengali_results}
\end{table*}


==> tables/main_results_validation_set.tex <==
\begin{table}[!t]
\label{tab:bengali_results_validation}
\centering
\begin{tabular}{l rrrr}
\toprule
\textbf{Model} & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}   \\
\midrule
 En2Bn-mBart  &  $0.05$ & $3.06$ & $0.20$ & $3.07$ \\
 OdiaGenAI-bn  & $0.00$ & $3.89$ & $0.00$ & $3.89$ \\
 TableLlama    & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
 GPT-3.5 & $1.14$ & $4.81$ & $1.67$ & $5.14$  \\
 GPT-4 & $0.00$ & $13.57$ & $5.43$ & $14.65$ \\
\midrule
\textbf{BnTQA-llama} & $9.41$ & $12.35$ & $9.85$ & $11.87$  \\
\textbf{BnTQA-mBart} & $\textbf{35.88}$ & $33.16$ & $\textbf{35.88}$ & $33.16$   \\
\textbf{BnTQA-M2M} & $28.05$ & $34.55$ & $28.05$ & $34.55$ \\ 
\bottomrule
\end{tabular}

\caption{Baseline and BanglaTabQA models' scores on Validation Set.}
\end{table}

==> tables/operator_classes.tex <==
\begin{table}[!h]
\small
\centering
\begin{tabular}{ll}
\toprule
\textbf{Operator class} & \textbf{Operations} \\
\midrule
arithmetic (A) & count, sum, average, max, min \\
sorting (So) & ascending, descending  \\
groupBy (G) & table column/row grouping  \\
filtering (F) & where, having \\
set (Se) & union, intersect, except \\
logical (L) & and, or, not, in, not in, between \\
\bottomrule
\end{tabular}
\caption{Classification of tableQA operations.}
\label{tab:operator_class}
\end{table}


==> tables/operator_classes_results_test_set.tex <==
\begin{table}[!t]
\centering
% \small
% \resizebox{1\columnwidth}{!}{
% \setlength{\tabcolsep}{0.7mm}
\begin{tabularx}{1\textwidth}{l@{~}cccc cccc}
\toprule
\multirow{2}{*}{\textbf{\makecell{Op}}} & \multicolumn{4}{c}{Validation set scores (\%)} & \multicolumn{4}{c}{Test set scores (\%)} \\
\cmidrule(r){2-5}
\cmidrule{6-9}
  & \textbf{Table} & \textbf{Row} & \textbf{Col} & \textbf{Cell} & \textbf{Table} & \textbf{Row} & \textbf{Col} & \textbf{Cell} \\
\midrule
A &  $65.79$ & $35.15$ & $65.79$ & $35.15$ &  $39.66$ & $55.64$ & $39.67$ & $55.64$  \\
So & $\textbf{74.86}$ & $70.63$ & $\textbf{75.14}$ & $68.03$ & $25.00$ & $25.00$ & $25.00$ & $25.00$ \\
G & $70.18$ & $78.84$ & $71.05$ & $78.84$ & $50.00$ & $76.92$ & $50.00$ & $76.92$   \\
F & $62.77$ & $70.59$ & $62.97$ & $70.64$  & $37.78$ & $35.86$ & $37.77$ & $35.86$ \\
Se  & $62.50$ & $\textbf{89.47}$ & $62.50$ & $\textbf{89.47}$ & $36.11$ & $49.10$ & $36.11$ & $49.10$  \\ 
L & $67.29$ & $65.19$ & $67.57$ & $65.40$ & $34.38$ & $13.23$ & $34.38$ & $13.23$  \\ 
\bottomrule
\end{tabularx}
% }
\caption{BnTQA-mBart scores on Operator classes.}
\label{tab:operator_results}
\end{table}


% \begin{table}[!t]
% \label{tab:operator_results_test_set}
% \centering
% \small
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{l@{~}cccc}
% \toprule
% \textbf{\makecell{Operator \\Class}} & \textbf{Table} & \textbf{Row} & \textbf{Col} & \textbf{Cell} \\
% \midrule
% arithmetic &   $39.66$ & $55.64$ & $39.67$ & $55.64$  \\
% sorting &  $25.00$ & $25.00$ & $25.00$ & $25.00$ \\
% groupBy &  $50.00$ & $76.92$ & $50.00$ & $76.92$   \\
% filtering  & $37.78$ & $35.86$ & $37.77$ & $35.86$ \\
% set  & $36.11$ & $49.10$ & $36.11$ & $49.10$  \\ 
% logical & $34.38$ & $13.23$ & $34.38$ & $13.23$  \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{BnTQA-mBart test scores on Operator classes.}
% \end{table}

==> tables/operator_classes_validation_set.tex <==
\begin{table}[!t]
\label{tab:operator_results_validation}
\centering
\small
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l@{~}cccc}
\toprule
\textbf{\makecell{Operator \\Class}} & \textbf{Table} & \textbf{Row} & \textbf{Col} & \textbf{Cell}  \\
\midrule
arithmetic &  $65.79$ & $35.15$ & $65.79$ & $35.15$  \\
sorting & $25.00$ & $25.00$ & $25.00$ & $25.00$ \\
groupBy & $50.00$ & $76.92$ & $50.00$ & $76.92$   \\
filtering &  $37.78$ & $35.86$ & $37.77$ & $35.86$ \\
set  &  $36.11$ & $49.10$ & $36.11$ & $49.10$  \\ 
logical &  $34.38$ & $13.23$ & $34.38$ & $13.23$  \\ 
\bottomrule
\end{tabular}
}
\caption{BnTQA-mBart validation set scores on Operator classes.}
\end{table}

==> tables/side_by_side.tex <==
\begin{table*}[!htb]
    \begin{minipage}{.45\linewidth}
     %  \centering
     %  \small
     %    \begin{tabular}{lp{9mm}p{5mm}p{5mm}p{5mm}r}
     %        \toprule
     %      \textbf{\makecell{Post-\\Proc\\-ess}} & \textbf{BnTQA} & \textbf{Tab} &  \textbf{Row} &  \textbf{Col} &  \textbf{Cell}  \\
     %        \midrule
     %     \multirow{3}{*}{No} &  -llama & $0.00$ & $0.00$ & \phantom{0}$0.00$ & $0.26$ \\ 
     %        & -mBart & $0.00$ & $8.70$ & $10.74$ & $8.70$ \\
     %        & -M2M & $0.00$ & $0.00$ & \phantom{0}$0.00$ & $0.00$ \\
     %        \midrule
     % \multirow{3}{*}{Yes}      & -llama & \phantom{0}$5.74$ & $17.59$ & \phantom{0}$5.69$ & $15.49$ \\ 
     %        & -mBart & $19.01$ & $20.74$ & $19.01$ & $20.74$ \\ 
     %        & -M2M & $18.18$ & $35.80$ & $18.18$ & $35.80$ \\
     %        \bottomrule
     %        \end{tabular}
            
     %    \caption{\makecell{Zero-shot cross-lingual \\transfer of\\ BanglaTabQA models on Hindi test set}}
     %    \label{tab:0_shot_cross_lingual}
    \small
    \centering
    \begin{tabular}{ll}
    \toprule
    \textbf{Operator class} & \textbf{Operations} \\
    \midrule
    arithmetic (A) & count, sum, average, max, min \\
    sorting (So) & ascending, descending  \\
    groupBy (G) & table column/row grouping  \\
    filtering (F) & where, having \\
    set (Se) & union, intersect, except \\
    logical (L) & and, or, not, in, not in, between \\
    \bottomrule
    \end{tabular}
    \caption{Classification of tableQA operations.}
    \label{tab:operator_class}
        
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \small
        \begin{tabular}{l@{~}p{7mm}p{7mm}p{7mm}p{7mm} p{7mm}p{7mm}p{7mm}p{7mm}}
            \toprule
            \multirow{2}{*}{\textbf{\makecell{Op}}} & \multicolumn{4}{c}{Validation set scores (\%)} & \multicolumn{4}{c}{Test set scores (\%)} \\
            \cmidrule(r){2-5}
            \cmidrule{6-9}
              & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell} & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell} \\
            \midrule
            A &  $65.79$ & $35.15$ & $65.79$ & $35.15$ &  $39.66$ & $55.64$ & $39.67$ & $55.64$  \\
            So & $\textbf{74.86}$ & $70.63$ & $\textbf{75.14}$ & $68.03$ & $25.00$ & $25.00$ & $25.00$ & $25.00$ \\
            G & $70.18$ & $78.84$ & $71.05$ & $78.84$ & $50.00$ & $76.92$ & $50.00$ & $76.92$   \\
            F & $62.77$ & $70.59$ & $62.97$ & $70.64$  & $37.78$ & $35.86$ & $37.77$ & $35.86$ \\
            Se  & $62.50$ & $\textbf{89.47}$ & $62.50$ & $\textbf{89.47}$ & $36.11$ & $49.10$ & $36.11$ & $49.10$  \\ 
            L & $67.29$ & $65.19$ & $67.57$ & $65.40$ & $34.38$ & $13.23$ & $34.38$ & $13.23$  \\ 
            \bottomrule
            \end{tabular}
            \caption{BnTQA-mBart scores on Operator (Op) classes.}
            \label{tab:operator_results}
    \end{minipage} 
\end{table*}

==> tables/side_by_side_firgure_table.tex <==
\begin{table*}[!htb]
    \begin{minipage}{.55\linewidth}
      \centering
      \small
      \setlength{\tabcolsep}{1.7mm}
        \begin{tabular}{lp{7mm}p{7mm}p{7mm}p{7mm} p{7mm}p{7mm}p{7mm}p{7mm}}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{Validation Set scores (\%)} & \multicolumn{4}{c}{Test Set scores (\%)} \\ 
    \cmidrule(r){2-5}
    \cmidrule{6-9}
     & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell}  & \textbf{Tab} & \textbf{Row} & \textbf{Col} & \textbf{Cell} \\
    \midrule
     En2Bn  &  $0.05$ & $3.06$ & $0.20$ & $3.07$ & $0.00$ & $4.73$ & $0.00$ & $4.73$\\
     OdiaG  & $0.00$ & $3.89$ & $0.00$ & $3.89$ & $0.69$ & $1.77$ & $0.69$ & $1.4$2 \\
     % TableLm  & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
     GPT-3.5 & $1.14$ & $4.81$ & $1.67$ & $5.14$ & $6.04$ & $10.06$ & $9.12$ & $9.84$ \\
     GPT-4 & $0.00$ & $13.57$ & $5.43$ & $14.65$ & $26.83$ & $\textbf{38.67}$ & $26.74$ & $\textbf{36.51}$ \\
    \midrule
    \textbf{BnTQA} & & & & & & & & \\
    \textbf{-llama} & $\textbf{60.08}$ & $\textbf{68.30}$ & $\textbf{60.47}$ & $\textbf{68.30}$ & $9.41$ & $12.35$ & $9.85$ & $11.87$  \\
    \textbf{-mBart} & $56.63$  & $64.1$ & $56.79$ & $64.31$ & $\textbf{35.88}$ & $33.16$ & $\textbf{35.88}$ & $33.16$   \\
    \textbf{-M2M} & $45.31$ & $58.07$ & $45.29$ & $58.04$ & $28.05$ & $34.55$ & $28.05$ & $34.55$ \\ 
    \bottomrule
    \end{tabular}
        \caption{Baseline and BanglaTabQA models' scores (\%).}
        \label{tab:bengali_results}
    \end{minipage}%
    \begin{minipage}{.55\linewidth}
      \centering
        \small
         \begin{tabular}{cp{7mm}p{7mm}p{7mm}p{7mm}}
    \toprule
   \textbf{Model} & \textbf{Tab} &  \textbf{Row} &  \textbf{Col} &  \textbf{Cell} \\
    \midrule
    OpHathi & $0.00$ & $0.11$ & $0.37$ & $0.74$\\
     GPT-3.5  & $8.20$ & $10.29$ & $7.10$ & $9.81$\\
     GPT-4  & $11.11$ & $21.49$ & $11.76$ & $20.84$\\
    \midrule
    \textbf{HiTQA} & & & \\
    \textbf{-llama} & \\
    \textbf{-mBart} & $28.93$ & $39.49$ & $28.93$ & $39.42$ \\
    \textbf{-M2M} & $-$ & $-$ & $-$ & $39.42$ \\
    \textbf{-BnTQA} & $\textbf{41.32}$ & $\textbf{47.26}$ & $\textbf{41.32}$ & $\textbf{47.26}$ \\
    \bottomrule
    \end{tabular}
    \label{tab:hitabqa}
    \caption{Scores (\%) of HindiTabQA \\models on Hindi test set.}
    \label{tab:hitabqa}
    \end{minipage} 
\end{table*}
